Thinking with Images as Continuous Actions: Numerical Visual Chain-of-Thought

Recent MLLMs increasingly rely on visual chain-of-thought to perform region-grounded reasoning over images. However, existing approaches ground regions via either textified coordinates (causing modality mismatch and semantic fragmentation) or fixed-granularity patches that both limit precise region selection and often require non-trivial architectural changes. In this paper, we propose Numerical Visual Chain-of-Thought (NV-CoT), a framework that enables MLLMs to reason over images using continuous numerical coordinates. NV-CoT expands the MLLM action space from discrete vocabulary tokens to a continuous Euclidean space, allowing models to directly generate bounding-box coordinates as actions with only minimal architectural modification. The framework supports both supervised fine-tuning and reinforcement learning. In particular, we replace categorical token policies with a Gaussian (or Laplace) policy over coordinates and introduce stochasticity via reparameterized sampling, making NV-CoT fully compatible with GRPO-style policy optimization. Extensive experiments on three benchmarks against 11 representative visual reasoning baselines demonstrate that NV-CoT significantly improves localization precision and final answer accuracy, while also accelerating training convergence, validating the effectiveness of continuous-action visual reasoning in MLLMs. Project page: https://kesenzhao.github.io/NV-CoT/

==> tables/bbox.tex <==
\centering
% \captionsetup{font=footnotesize,skip=2pt}
\captionof{table}{Bounding-box IoU on the Vis-CoT-363K dataset. \ours~substantially improves localization precision over Vis-CoT, with the $\ell_1$ loss outperforming the $\ell_2^2$ loss.}\label{tab:IoU}\label{table:bbox}
{\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccc}
\toprule[1pt]
 & Vis-CoT & \ours~($\ell_2^2$) & \ours~($\ell_1$)  \\ \midrule
Bbox IoU & 47.3 & 57.4 & 59.5\\ \bottomrule[1pt]
\end{tabular}
\par}
